Vision Function Layer in Multimodal LLMs

This study identifies that visual-related functional decoding is distributed across different decoder layers in Multimodal Large Language Models (MLLMs). Typically, each function, such as counting, grounding, or OCR recognition, narrows down to two or three layers, which we define as Vision Function Layers (VFL). Additionally, the depth and its order of different VFLs exhibits a consistent pattern across different MLLMs, which is well-aligned with human behaviors (e.g., recognition occurs first, followed by counting, and then grounding). These findings are derived from Visual Token Swapping, our novel analytical framework that modifies targeted KV cache entries to precisely elucidate layer-specific functions during decoding. Furthermore, these insights offer substantial utility in tailoring MLLMs for real-world downstream applications. For instance, when LoRA training is selectively applied to VFLs whose functions align with the training data, VFL-LoRA not only outperform full-LoRA but also prevent out-of-domain function forgetting. Moreover, by analyzing the performance differential on training data when particular VFLs are ablated, VFL-select automatically classifies data by function, enabling highly efficient data selection to directly bolster corresponding capabilities. Consequently, VFL-select surpasses human experts in data selection, and achieves 98% of full-data performance with only 20% of the original dataset. This study delivers deeper comprehension of MLLM visual processing, fostering the creation of more efficient, interpretable, and robust models.

==> table/benchmark_t5.tex <==
\begin{table*}[t]
    
    \centering
    % Removed the incorrect \sisetup{ V/} line
    \resizebox{\textwidth}{!}{% Use % to avoid spurious space
        \begin{tabular}{l | c % SQA-I kept as 'c' due to special format
                         S[table-format=2.1] | % MMMU
                         S[table-format=2.1] | % POPE
                         S[table-format=2.1] | % CVBench
                         S[table-format=2.1]  % TextVQA
                        }
            \toprule
            \multicolumn{1}{c|}{}   & \multicolumn{2}{c|}{\textbf{General \& Knowledge}} & \multicolumn{1}{c|}{\textbf{Recognition}} & \multicolumn{1}{c|}{\textbf{Spatial}} & \textbf{OCR}   \\
            {\textbf{Vision Encoder \& Language Model}}  & {{SQA-I~\cite{scienceqa}}}  & {{MMMU~\cite{yue2023mmmu}}} & {{POPE~\cite{pope}}}  &  {{CVBench~\cite{tong2024cambrian}}} & {{ChartQA~\cite{masry2022chartqa}}}\\
            \midrule
            CLIP~\cite{radford2021learning} \& Vicuna~\cite{zheng2023judging}-7B & 68.8  & 34.7  &  86.4   & 56.2  & 22.0 \\
            \hspace{1em}\textit{-- drop 8 v-layers}  & 68.8  &  34.4  & 86.4   & 56.4   & \numreddownv{21.0} \\
            \hspace{1em}\textit{-- drop 16 v-layers}  & 68.7  & 34.3   & 86.0  &  \numreddownv{53.7} &  \numreddowndownv{\underline{\underline{15.9}}} \\
            \hspace{1em}\textit{-- drop 20 v-layers} & 69.0  &  35.2 & \numreddownv{83.2} & \numreddowndownv{\underline{\underline{43.0}}}   & 13.8 \\
            \hspace{1em}\textit{-- drop 24 v-layers}  & \numreddownv{65.7}  & \numreddownv{33.9}   & \numreddowndownv{\underline{\underline{38.1}}} & 37.2   & 12.8 \\
            \midrule
            CLIP~\cite{radford2021learning} \& Vicuna~\cite{zheng2023judging}-13B  & 72.7  & 35.4 & 85.9  & 53.0  & 22.6 \\
            \hspace{1em}\textit{-- drop 8 v-layers}  & 72.6  &  35.8  & 86.0   & 53.2 & \numreddownv{21.1} \\
            \hspace{1em}\textit{-- drop 16 v-layers}  & 72.7  & 35.4  & 84.9  &  53.2  &  \numreddowndownv{\underline{\underline{15.8}}} \\
            \hspace{1em}\textit{-- drop 20 v-layers}  & 72.2  & 37.2   & \numreddownv{74.9}   & \numreddownv{51.2} & 15.0 \\
            \hspace{1em}\textit{-- drop 24 v-layers}  & \numreddownv{70.1}  & \numreddownv{34.6}   & \numreddowndownv{\underline{\underline{11.5}}}  & 52.2 & 13.5 \\
            \midrule


            DINOv2~\cite{oquab2023dinov2} \& LLaMA-3~\cite{grattafiori2024llama}-8B & 71.4  & 32.7  &  85.5   & 64.8  & 73.1 \\
            \hspace{1em}\textit{-- drop 8 v-layers}  & 70.1  &  34.0  & 85.0   & 66.4   & \numreddownv{70.8} \\
            \hspace{1em}\textit{-- drop 16 v-layers}  & 70.5  & 31.3   & 84.5  &  68.9 &  \numreddowndownv{\underline{\underline{18.6}}} \\
            \hspace{1em}\textit{-- drop 20 v-layers} & 69.6  &  34.8 & \numreddownv{78.2} & \numreddownv{66.5}   & 13.4 \\
            \hspace{1em}\textit{-- drop 24 v-layers}  & \numreddownv{67.7}  & 36.5   & \numreddowndownv{\underline{\underline{6.6}}} & \numreddowndownv{\underline{\underline{44.3}}}   & 11.6 \\
            \midrule

            %%% TAG
            DINOv2~\cite{oquab2023dinov2} \& Vicuna~\cite{zheng2023judging}-13B  & 74.3  & 37.7 & 85.6  & 65.4  & 72.7 \\
            \hspace{1em}\textit{-- drop 8 v-layers}  & 74.3  &  40.7  & 84.6   & 66.0 & \numreddownv{62.0} \\
            \hspace{1em}\textit{-- drop 16 v-layers}  & 74.3  & 37.4  & 84.9  &  66.2  &  \numreddowndownv{\underline{\underline{17.8}}} \\
            \hspace{1em}\textit{-- drop 20 v-layers}  & 74.6  & 37.2   & \numreddownv{76.9}   & \numreddownv{57.3} & 14.0 \\
            \hspace{1em}\textit{-- drop 24 v-layers}  & \numreddownv{72.4}  & \numreddownv{36.6}   & \numreddowndownv{\underline{\underline{17.6}}}  & 51.0 & 13.1 \\
            \midrule

            
            Qwen-ViT \& Qwen2.5-LM~\cite{bai2023qwen}-3B  & 80.3  & 46.3  & 87.0  & 72.9  & 83.4 \\
            \hspace{1em}\textit{-- drop 4 v-layers} & 80.0 & 46.9  & 86.9 & 72.9&  \numreddowndownv{\underline{\underline{78.6}}} \\
            \hspace{1em}\textit{-- drop 8 v-layers} & 80.1 & 46.5   & 86.9   &72.6  & 60.0 \\
            \hspace{1em}\textit{-- drop 16 v-layers} & 79.6 &  46.2  & \numreddownv{82.7}  & \numreddowndownv{\underline{\underline{56.4}}} & 13.0 \\
            \hspace{1em}\textit{-- drop 20 v-layers} & \numreddownv{76.7} & \numreddownv{45.2} & \numreddowndownv{\underline{\underline{19.4}}}   & 47.2 & 13.2 \\
            \midrule
            Qwen-ViT \& Qwen2.5-LM~\cite{bai2023qwen}-7B  & 87.2  & 50.7  & 86.1   & 80.8   & 83.2 \\
            % \hspace{1em}\textit{-- drop 4 v-layers} & 83.5 & 48.0 & 1698.7 & 86.5 & 77.1 & & 84.1 & 85.3 &88.1 & 86.3  \\
            \hspace{1em}\textit{-- drop 4 v-layers} & 87.4 & 50.8  & 86.3   & 81.0 &  \numreddowndownv{\underline{\underline{82.7}}}  \\
            \hspace{1em}\textit{-- drop 8 v-layers} & 87.4 & 50.6  & 86.2   & 80.6 & 20.5  \\
            \hspace{1em}\textit{-- drop 12 v-layers} & 87.2 & 50.2  & \numreddownv{79.5}   & \numreddowndownv{\underline{\underline{69.1}}} & 17.4  \\
            \hspace{1em}\textit{-- drop 18 v-layers} & \numreddownv{77.3} & \numreddowndownv{\underline{\underline{45.8}}}  & \numreddowndownv{\underline{\underline{37.1}}}  & 44.2 & 14.3  \\
            \bottomrule
        \end{tabular}
    }% End resizebox
    \caption{\textbf{Vision Token Dropping on General Benchmarks.} 
    \numreddownv{A} indicates the onset of performance degradation, while \numreddowndownv{\underline{\underline{A}}} highlights significant drops. The results reveal a consistent hierarchical order of vision function layers across diverse MLLMs. 
}

\label{tab:main-intro-drop} % Changed label slightly to avoid potential conflict if tab:main-intro used elsewhere
\end{table*}
